Procedural Adherence and Interpretability Through Neuro-Symbolic Generative Agents

The surge in popularity of large language models (LLMs) has opened doors for new approaches to the creation of interactive agents. However, managing and interpreting the temporal behavior of such agents over the course of a potentially infinite interaction remain challenging. The stateful, long-term horizon reasoning required for coherent agent behavior does not fit well into the LLM paradigm. We propose a combination of formal logic-based program synthesis and LLM content generation to bring guarantees of procedural adherence and interpretability to generative agent behavior. To illustrate the benefit of procedural adherence and interpretability, we use Temporal Stream Logic (TSL) to generate an automaton that enforces an interpretable, high-level temporal structure on an agent. With the automaton tracking the context of the interaction and making decisions to guide the conversation accordingly, we can drive content generation in a way that allows the LLM to focus on a shorter context window. We evaluated our approach on different tasks involved in creating an interactive agent specialized for generating choose-your-own-adventure games. We found that over all of the tasks, an automaton-enhanced agent with procedural guarantees achieves at least 96% adherence to its temporal constraints, whereas a purely LLM-based agent demonstrates as low as 14.67% adherence.

==> figs/sys.tex <==
\begin{figure}
  \centering
  \begin{tikzpicture}[scale=1]
\newcommand{\arrow}[3]{
  \node[anchor=west,inner sep=0pt] at #1 (#2) {
    \begin{tikzpicture}[scale=0.8,inner sep=2pt]
      \node[arrow] (A) at (-3,0) {#3};
      \fill[green!10] (A.south east) -- (A.south west) --
      (A.north west) -- (A.north east)
      -- ($ (A.east) + (0.2,0) $) -- cycle;
      \node[arrow] (A) at (-3,0) {\phantom{#3}};
      \draw (A.south east) -- (A.south west) --
      (A.north west) -- (A.north east) --
      ($ (A.east) + (0.2,0) $) -- cycle;
      \node[text depth=0pt] at (A) at (-3,0) {#3};
    \end{tikzpicture}
  };
}

    \node[anchor=east,inner sep=0pt] at (-2.4,-0.8) {
      \small
      \begin{tabular}{c}
        input: \\ $summary$
      \end{tabular}
    };
    
    \node[anchor=west,inner sep=0pt] at (2.05,0.1) {
      \small
      \begin{tabular}{c}
        output: \\
        $ storyPassage $
      \end{tabular}
    };

    \node at (0,0) {
      \begin{tikzpicture}[xscale=0.8,yscale=0.56]
        \node[draw=black, drop shadow, fill=gray!10,minimum height=6.6em, minimum width=12em] (C) {};

        \node[rounded corners, draw=black, drop shadow, fill=yellow!10,minimum height=2.5em] (control) at (1.5,-1.1) {
          \small
          \begin{tabular}{c}
            control \\ circuit
          \end{tabular}
        };

        % predicates 
        \arrow{(-2.2,-0.6)}{p1}{$ \name{inCave} $};
        \arrow{(-2.2,-1.6)}{p2}{$ \name{inMarket} $};
        % \arrow{(-2.2, 0.4)}{p3}{$ \name{inTown} $};
        
        % functions
        
        \arrow{(-0.50, 1.50)}{u1}{$ \name{toMarket} $};
        \arrow{(-0.05, 1.00)}{u2}{$ \name{toCave} $};
        % \arrow{(0.20, 1)}{u3}{$ \name{toTown} $};

        % signals
        \path[->,>=stealth,line width=0.7pt]
	let 
	  \p1 = (p1.west),
	  \p2 = (p2.west)
	in
        ($ (C.west) + (-0.6,\y2) $) edge ($ (C.west) + (0,\y2) $)
        ($ (C.east) + (0,0.5) $) edge ($ (C.east) + (0.6,0.5) $)
        ;

        % internal signals for predicates
        \path[->,>=stealth,line width=0.7pt,gray]
	let 
	  \p1 = (p1.west),
	  \p2 = (p2.west),
	  \p3 = (p1.east),
	  \p4 = (p2.east),
	  \p5 = (control.west)
	in
        ($ (C.west) + (0,\y2) $) edge ($ (p2.west) $)
        ($ (p2.east) $) edge ($ (\x5, \y4) $)
        ;

         \path[->,>=stealth,line width=0.7pt,gray]
	let 
	  \p1 = (p1.west),
	  \p2 = (p2.west)
	in
        ($ (control.north) + (-0.13, 0.0) $) edge ($ (u2.south) + (0.4, 0.0) $)
        ;

        \path[->,>=stealth,line width=0.7pt,gray,draw]
        let
	  \p2 = (p2.west)
        in
        ($ (C.west) + (0,\y2) $) -- ($ (C.west) + (0.1,\y2) $) |- ($ (p1.west) + (0, -0.2)$);

        \path[->,>=stealth,line width=0.7pt,gray,draw]
        let
	  \p2 = (p3.east),
        \p1 = (p2.east)
        in
        % ($ (\x2, \y2) $) -- ($ (0.0, \y2) $) |- ($ (control.west) + (0, 0.6) $);

        \path[->,>=stealth,line width=0.7pt,gray,draw]
        let
	  \p2 = (p3.west)
        in
        % ($ (C.west) + (0.1,\y2) $) -- ($ (C.west) + (0.1,\y2) $) |- ($ (p3.west) + (0, -0.2)$);

        \path[->,>=stealth,line width=0.7pt,gray,draw]
        let
	  \p2 = (p1.east)
        in
        ($ (\x2, \y2) $) -- ($ (-0.1,\y2) $) |- ($ (control.west) + (0, 0.05)$);

        \path[->,>=stealth,line width=0.7pt,gray,draw]
        let
	  \p2 = (p2.west)
        in
        ($ (C.west) + (0.1,\y2) $) |- ($ (u1.west) + (0, -0.3)$);

        \path[->,>=stealth,line width=0.7pt,gray,draw]
        let 
          \p1 = (u2.east),
          \p2 = (C.east)
        in
        ($ (u2.east) $) to[-|-] ($ (\x2, \y1) + (0, -0.51) $);

      \end{tikzpicture}
    };
  \end{tikzpicture}
  \caption{A visualisation of the system described by the TSL spec in Fig.~\ref{fig:adventure}. The system uses predicate evaluations on the story summary to control which function will be applied to generate the updated story passage in each time step.}
  \label{fig:sys}
\end{figure}

